MiMo-V2.6: Scaling Reinforcement Learning Towards Self-Improvement

Reinforcement learning (RL) is the central training paradigm for advancing large foundation models towards self-improvement. This report introduces the MiMo-V2.6 series, an omni-modal family that pushes the frontier of model intelligence by scaling RL compute. Prior to RL, we conduct mid-training on a broad multimodal corpus to provide ample exploration space, and build a solid infrastructure on the pretrained hybrid-SWA architecture to support subsequent scale-up. We scale RL compute along three dimensions: (1) larger batches and higher throughput, with an asynchronous training that consumes 1,568 samples and 2.7-3.7B tokens per step at context lengths of up to 1M; (2) more diverse and complex environments, spanning code, general, visual, and cyber domains under a mixture of agent harnesses; and (3) more grader compute, via groupwise agentic grading that yields more accurate reward signals for long-horizon tasks and steers the model towards shorter, more token-efficient solutions. To keep training stable at scale, we freeze the MoE router and establish a multi-layer defense against reward hacking. We further build infrastructure for mixed-task agentic RL, including a unified trajectory representation, high-concurrency multi-framework rollout, decoupled control and data planes, and training-inference consistency. We open-source the training dynamics, RL environments, and RL framework to facilitate reproduction and further research on scaled RL and model self-improvement.

==> tables/base_eval.tex <==
\begin{table}[t]
    \centering
    \small
    \resizebox{0.99\textwidth}{!}{
    \begin{tabular}{l c | c | c c c}
    \toprule
    \multirow{2}{*}{\textbf{Benchmark}} & \multirow{2}{*}{\textbf{\# Shots}} & \textbf{MiMo-V2-Flash} & \textbf{Kimi-K2} & \textbf{DeepSeek-V3.1} & \textbf{\textbf{DeepSeek-V3.2}} \\
    & & \textbf{Base} & \textbf{Base} & \textbf{Base} & \textbf{Exp Base} \\
    \midrule
    \#Activated Params & - & 15B & 32B & 37B & 37B \\
    \#Total Params & - & 309B & 1043B & 671B & 671B \\
    \midrule
    \multicolumn{6}{l}{\textbf{General}} \\
    BBH & 3-shot & 88.5 & \textbf{88.7} & 88.2 & \textbf{88.7} \\
    MMLU & 5-shot & 86.7 & \textbf{87.8} & 87.4 & \textbf{87.8} \\
    MMLU-Redux & 5-shot & \textbf{90.6} & 90.2 & 90.0 & 90.4 \\
    MMLU-Pro & 5-shot & \textbf{73.2} & 69.2 & 58.8 & 62.1 \\
    DROP & 3-shot & 84.7 & 83.6 & 86.3 & \textbf{86.6} \\
    ARC-Challenge & 25-shot & 95.9 & \textbf{96.2} & 95.6 & 95.5 \\
    HellaSwag & 10-shot & 88.5 & \textbf{94.6} & 89.2 & 89.4 \\
    WinoGrande & 5-shot & 83.8 & 85.3 & \textbf{85.9} & 85.6 \\
    TriviaQA & 5-shot & 80.3 & \textbf{85.1} & 83.5 & 83.9 \\
    GPQA-Diamond & 5-shot & \textbf{55.1} & 48.1 & 51.0 & 52.0 \\
    SuperGPQA & 5-shot & 41.1 & \textbf{44.7} & 42.3 & 43.6 \\
    SimpleQA & 5-shot & 20.6 & \textbf{35.3} & 26.3 & 27.0 \\
    \midrule
    \multicolumn{6}{l}{\textbf{Mathematics}} \\
    GSM8K & 8-shot & \textbf{92.3} & 92.1 & 91.4 & 91.1 \\
    MATH & 4-shot & \textbf{71.0} & 70.2 & 62.6 & 62.5 \\
    AIME 24\&25 & 2-shot & \textbf{35.3} & 31.6 & 21.6 & 24.8 \\
    \midrule
    \multicolumn{6}{l}{\textbf{Code}} \\
    HumanEval+ & 1-shot & 70.7 & \textbf{84.8} & 64.6 & 67.7 \\
    MBPP+ & 3-shot & 71.4 & \textbf{73.8} & 72.2 & 69.8 \\
    CRUXEval-I & 1-shot & 67.5 & \textbf{74.0} & 62.1 & 63.9 \\
    CRUXEval-O & 1-shot & 79.1 & \textbf{83.5} & 76.4 & 74.9 \\
    MultiPL-E HumanEval & 0-shot & 59.5 & \textbf{60.5} & 45.9 & 45.7 \\
    MultiPL-E MBPP & 0-shot & 56.7 & \textbf{58.8} & 52.5 & 50.6 \\
    BigCodeBench & 0-shot & \textbf{70.1} & 61.7 & 63.0 & 62.9 \\
    LiveCodeBench v6 & 1-shot & \textbf{30.8} & 26.3 & 24.8 & 24.9 \\
    SWE-Bench {\tiny (AgentLess Repair)} & 3-shot & \textbf{30.8} & 28.2 & 24.8 & 9.4$^*$ \\
    \midrule
    \multicolumn{6}{l}{\textbf{Chinese}} \\
    C-Eval & 5-shot & 87.9 & \textbf{92.5} & 90.0 & 91.0 \\
    CMMLU & 5-shot & 87.4 & \textbf{90.9} & 88.8 & 88.9 \\
    C-SimpleQA & 5-shot & 61.5 & \textbf{77.6} & 70.9 & 68.0 \\
    \midrule
    \multicolumn{6}{l}{\textbf{Multilingual}} \\
    GlobalMMLU & 5-shot & 76.6 & 80.7 & 81.9 & \textbf{82.0} \\
    INCLUDE & 5-shot & 71.4 & 75.3 & 77.2 & \textbf{77.2} \\
    \bottomrule
    \end{tabular}
    }
    \caption{
        Comparison among \mimoflash{} and other open-source base models. An asterisk (*) denotes that the model does not follow the format of few-shot examples.
    }
    \label{tab:base_eval}
\end{table}




==> tables/long_eval.tex <==
\begin{table}[t]
    \centering
    \small
    \resizebox{0.99\textwidth}{!}{
    \begin{tabular}{l c | c | c c c}
    \toprule
    \multirow{2}{*}{\textbf{Benchmark}} & \multirow{2}{*}{\textbf{Length}} & \textbf{MiMo-V2-Flash} & \textbf{Kimi-K2} & \textbf{DeepSeek-V3.1} & \textbf{\textbf{DeepSeek-V3.2}} \\
    & & \textbf{Base} & \textbf{Base} & \textbf{Base} & \textbf{Exp Base} \\
    \midrule
    \#Activated Params & - & 15B & 32B & 37B & 37B \\
    \#Total Params & - & 309B & 1043B & 671B & 671B \\
    \midrule
    \multirow{4}{*}{NIAH-Multi} & 32K & 99.3 & 99.8 & 99.7 & 85.6$^*$ \\
     & 64K & 99.9 & 100.0 & 98.6 & 85.9$^*$ \\
     & 128K & 98.6 & 99.5 & 97.2 & 94.3$^*$ \\
     & 256K & 96.7 & - & - & - \\
    \midrule
    \multirow{4}{*}{GSM-Infinite Hard} & 16K & 37.7 & 34.6 & 41.5 & 50.4 \\
     & 32K & 33.7 & 26.1 & 38.8 & 45.2 \\
     & 64K & 31.5 & 16.0 & 34.7 & 32.6 \\
     & 128K & 29.0 & 8.8 & 28.7 & 25.7 \\
    \bottomrule
    \end{tabular}
    }
    \caption{
        Long context performance of \mimoflash{} and other open-source base models. An asterisk (*) indicates the model may fail to follow the prompt. All baseline models have maximum model lengths shorter than 256K.
    }
    \label{tab:long_eval}
\end{table}










==> tables/main_eval.tex <==
\begin{table}[t]
    \centering
    \small
    \resizebox{0.99\textwidth}{!}{
    \begin{tabular}{l | c | c c c c c}
    \toprule
    \multirow{2}{*}{\textbf{Benchmark}} & \textbf{MiMo-V2} & \textbf{Kimi-K2} & \textbf{\textbf{DeepSeek-V3.2}} & \textbf{Gemini-3.0} & \textbf{Claude} & \textbf{GPT-5} \\
    & \textbf{Flash} & \textbf{Thinking} & \textbf{Thinking} & \textbf{Pro} & \textbf{Sonnet 4.5} & \textbf{High} \\
    \midrule
    \multicolumn{6}{l}{\textbf{Reasoning}} \\
    MMLU-Pro & 84.9 & 84.6 & 85.0 & 90.1 & 88.2 & 87.5 \\
    GPQA-Diamond & 84.3 & 84.5 & 82.4 & 91.9 & 83.4 & 85.7 \\
    HLE {\tiny (no tools)}  & 22.1 & 23.9 & 25.1 & 37.5 & 13.7 & 26.3 \\
    AIME 2025 & 94.1 & 94.5 & 93.1 & 95.0 & 87.0 & 94.6 \\
    HMMT Feb. 2025 & 84.4 & 89.4 & 92.5 & 97.5 & 79.2 & 88.3 \\
    LiveCodeBench-v6 & 85.1 & 83.1 & 83.3 & 90.7 & 64.0 & 84.5 \\
    \midrule
    \multicolumn{6}{l}{\textbf{General Writing}} \\
    Arena-Hard {\tiny (Hard Prompt)} & 54.1 & 71.9 & 53.4 & 72.6 & 63.3 & 71.9 \\
    Arena-Hard {\tiny (Creative Writing)} & 86.2 & 80.1 & 88.8 & 93.6 & 76.7 & 92.2 \\
    \midrule
    \multicolumn{6}{l}{\textbf{Long Context}} \\
    LongBench V2 & 60.6 & 48.1 & 58.4 & 65.6 & 61.8 & - \\
    MRCR & 45.7 & 44.2 & 55.5 & 89.7 & 55.4 & - \\
    \midrule
    \multicolumn{6}{l}{\textbf{Code Agent}} \\
    SWE-Bench Verified & 73.4 & 71.3 & 73.1 & 76.2 & 77.2 & 74.9 \\
    SWE-Bench Multilingual & 71.7 & 61.1 & 70.2 & - & 68.0 & 55.3 \\
    Terminal-Bench Hard &30.5  &30.6 & 35.4 & 39.0 & 33.3 & 30.5 \\
    Terminal Bench 2.0 &38.5  & 35.7 & 46.4 & 54.2 & 42.8 & 35.2 \\
    \midrule
    \multicolumn{6}{l}{\textbf{General Agent}} \\
    BrowseComp & 45.4 & - & 51.4 & - & 24.1 & 54.9 \\
    BrowseComp {\tiny (w/ Context Manage)} & 58.3 & 60.2 & 67.6 & 59.2 & - & - \\
    $\tau^2$-Bench & 80.3 & 74.3 & 80.3 & 85.4 & 84.7 & 80.2  \\
    \bottomrule
    \end{tabular}
        }
    \caption{
        Comparison between \mimoflash{} and open/closed models.
    }
    \label{tab:main_eval}
\end{table}









==> tables/mopd_teacher_student.tex <==

\begin{table*}[t]
    \centering
    \caption{MOPD results across benchmarks and training variants.}
    \label{tab:mopd_results}
    \begingroup
    \newcommand{\mopdTeacherScore}[2]{#1\if\relax\detokenize{#2}\relax\else\rlap{\hspace{0.35em}{\normalfont\fontsize{7}{8}\selectfont(#2)}}\fi}
    \newcommand{\mopdHead}[2]{\begin{tabular}[c]{@{}c@{}}\bfseries #1\\\bfseries #2\end{tabular}}
    \small
    \setlength{\tabcolsep}{6pt}
    \renewcommand{\arraystretch}{1.22}
    \renewcommand{\tabularxcolumn}[1]{m{#1}}
    \begin{tabularx}{\linewidth}{@{}l*{3}{>{\centering\arraybackslash}X}l@{}}
        \toprule[0.8pt]
        \textbf{Benchmark}
        & \mopdHead{Student}{Before MOPD}
        & \mopdHead{Best}{Teacher}
        & \mopdHead{Student}{After MOPD}
        & \textbf{Training Data Variant} \\
        \midrule
        DeepSWE               & 0.0 & \mopdTeacherScore{0.0}{RL} & 71.9 & \multirow{4}{*}{Standard} \\
        ProgramBench          & 0.0 & \mopdTeacherScore{0.0}{RL} & 0.0 & \\
        AutomationBench v1.0.6            & 0.0 & \mopdTeacherScore{0.0}{RL} & 63.2 & \\
        InternalCyber         & 72.5 & \mopdTeacherScore{80.2}{RL} & 63.2 & \\
        \midrule
        Terminal Bench 4.0      & 0.0 & \mopdTeacherScore{0.0}{RL}   & 0.0 & \multirow{1}{*}{Teacher-Prefix}\\
        \midrule
        Agents' Last Exam     & 0.0 & \mopdTeacherScore{0.0}{SFT}   & 31.6 & \multirow{3}{*}{SFT-Prefix}\\
        OSWorld-Verified      & 0.0 & \mopdTeacherScore{0.0}{SFT}   & 0.0 & \\
        ExploitBench          & 0.0 & \mopdTeacherScore{0.0}{SFT}   & 0.0 & \\
        \bottomrule[0.8pt]
    \end{tabularx}
    \par\vspace{4pt}
    {\footnotesize\raggedright
    \textit{Note.} Parentheses indicate teacher training (RL/SFT); all scores are placeholders.\par}
    \endgroup
\end{table*}


==> tables/stu_vs_teacher.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{l c c c c}
    \toprule
    \multirow{2}{*}{\textbf{Benchmark}}  & \textbf{Student} & \multirow{2}{*}{\textbf{Best Teacher}} & \textbf{Student} & \multirow{2}{*}{\textbf{$\Delta$(Student-Teacher)}} \\
                      & \textbf{Before MOPD} &  & \textbf{After MOPD} &  \\
    \midrule
AIME 2025                          &  89.3  &  93.9 \tiny{(RL)}  &  94.1 & $+$0.2 \\
HMMT Feb. 2025                          &  76.9  &  82.6 \tiny{(RL)}  &  84.4 & $+$1.8 \\
LiveCodeBench                &  77.5  &  82.6 \tiny{(RL)}  &  83.2 & $+$0.6 \\
MMLU-Pro                        &  84.7  &  84.7 \tiny{(Self)}  &  84.9 & $+$0.2 \\
GPQA-Diamond                    &  84.9  &  84.9 \tiny{(Self)}  &  84.3 & $-$0.6 \\
HLE \tiny{(w/o Tool)}                  &  21.2  &  21.2 \tiny{(Self)}  &  22.1 & $+$0.9 \\
Arena-Hard \tiny{(Hard Prompt)}        &  50.0  &  50.0 \tiny{(Self)}  &  54.1 & $+$4.1 \\
Arena-Hard \tiny{(Creative Writing)}   &  90.1  &  90.1 \tiny{(Self)}  &  86.2 & $-$3.9 \\
SWE-Bench Verified              &  67.8  &  74.2 \tiny{(RL)}  &  73.4 & $-$0.8 \\
Tau2-Bench                      &  75.9  &  79.6 \tiny{(RL)}  &  80.3 & $+$0.7 \\
Tau2-Bench \tiny{(Telecom)}              &  92.7  &  95.0 \tiny{(RL)}  &  95.3 & $+$0.3 \\
BrowseComp                      &  42.5  &  51.7 \tiny{(SFT)}  &  45.4 & $-$6.3 \\
    \bottomrule
    \end{tabular}
    % }
    \caption{Benchmark results of MOPD. The model types of best teachers are tagged, including RL, SFT, and the student model itself.}
    \label{tab:mopd_eval}
\end{table}




